The Ad Types Problem

The Ad Types Problem (without gap rules) is a special case of the assignment problem in which there are $k$ types of nodes on one side (the ads), and an ordered set of nodes on the other side (the slots). The edge weight of an ad $i$ of type $\theta$ to slot $j$ is $v_i\cdot \alpha^{\theta}_j$ where $v_i$ is an advertiser-specific value and each ad type $\theta$ has a discount curve $\alpha^{(\theta)}_{1} \ge \alpha^{(\theta)}_{2} \ge ... \ge 0$ over the slots that is common for ads of type $\theta$. We present two contributions for this problem: 1) we give an algorithm that finds the maximum weight matching that runs in $O(n^2(k + \log n))$ time for $n$ slots and $n$ ads of each type---cf. $O(kn^3)$ when using the Hungarian algorithm---, and 2) we show to do VCG pricing in asymptotically the same time, namely $O(n^2(k + \log n))$, and apply reserve prices in $O(n^3(k + \log n))$. The Ad Types Problem (with gap rules) includes a matrix $G$ such that after we show an ad of type $\theta_i$, the next $G_{ij}$ slots cannot show an ad of type $\theta_j$. We show that the problem is hard to approximate within $k^{1- \epsilon}$ for any $\epsilon > 0$ (even without discount curves) by reduction from Maximum Independent Set. On the positive side, we show a Dynamic Program formulation that solves the problem (including discount curves) optimally and runs in $O(k\cdot n^{2k + 1})$ time.

==> extra-results-discounts-only.tex <==
\section{Additional Results for Discounts-only Setting}
\label{sec:extra-results-discounts-only}


\begin{lemma}
	For $k = 2$ ad types, there is a Dynamic Program that finds the optimal allocation in $O(m^2)$ time and space, provided the discount curves are monotonically decreasing.
\end{lemma}
\begin{proof}
	Let $v_1^{(1)}\geq v_2^{(1)} \geq ... \geq v_n^{(1)}$ be the ads of type $\theta_1$ is descending order, and $v_1^{(2)}\geq v_2^{(2)} \geq ... \geq v_n^{(2)}$ be the ads of type $\theta_2$ is descending order. Let $A$ be the DP table where $A_{i,j}$ is the value of the optimal allocation of the remaining ads to the remaining slots when we've assigned the first $i$ ads of type $\theta_1$ and the first $j$ slots of $\theta_2$, to the first $i + j$ slots.
	
	The recursion is that $A[i, j] = \max(\alpha_{i+j}^{(1)}\cdot v_{i+1}^{(1)}  + A_{i+1, j} ,\hspace{8px} \alpha_{i+j}^{(2)}\cdot v_{j+1}^{(2)}  + A_{i, j+1})$ and the base case is for $i, j$ such that $i+j \geq m+1$, we have $A_{i, j} = 0$.
	
	It's clear that the table can be generated in constant time per entry, and the table is triangular with $\binom{m}{2} = O(m^2)$ entries.
	
	
	Correctness. Claim: The ads of the same type, have to appear in descending order. Pf. Exchange argument. Using this, the correctness follows.
\end{proof}



\begin{lemma}
	If we initialize the Hungarian Algorithm by setting the dual variable for the advertisers to $0$ and the dual variables for the slots to $p_i = \max_j v_{ij}$, and we start each phase with an unmatched slot, the after each phase we have the market solution for if the unmatched slots didn't exist.
\end{lemma}
\begin{proof}[Proof sketch.]
	It's sufficient if the price of the unmatched slots is at least as high as the value that unmatched advertisers have for it.
	
	This is true during initialization, so it's sufficient if this is maintained during each phase.
	
	When we start with an unmatched slot during a phase, the during the adapted BFS, we only use matched edges to go from advertisers to slots. Therefore we'll never expand to another unmatched slot in a phase, and thus we won't update their prices.
	
	Since the prices of unmatched slots aren't updated until we start matching them in a phase of the Hungarian Algorithm, at the end of each phase, all unmatched slots are not selected in the market solution. QED.
\end{proof}

==> greedy-app.tex <==
% !TEX root = main.tex

\section{Greedy 2-approximation}
\label{sec:greedy-app}

In practice, running the Hungarian algorithm for dozens of slots and hundreds of ads can become prohibitive (due to stringent time constraints), so a common solution is to run a greedy algorithm. Starting from the empty matching, the algorithm picks the edges with maximum value, among the edges that are compatible with the matching we have so far. Given the structure of the discount curves, the algorithm will match the slots in descending order and will match the ads within the same type in decreasing order as well. Therefore, by keeping track of the highest unassigned slot and ad for each type, the algorithm can be implemented to run in $O(kn)$ time. Unfortunately, although fast, there are instances of the ad types problem where the algorithm can only recover half of the maximum social welfare.f
On the upside, the greedy algorithm actually \emph{is} guaranteed obtain at least half of the social welfare \cite{KVV90}, and the corresponding allocation function is also monotone so we can compute Myerson prices in $O(n^2)$ time.

\begin{proposition}
	The greedy algorithm is a $2$-approximation for the Ad Types problem without gap rules and this is tight.
\end{proposition}

\begin{proof}
	The upper bound on the performance of greedy follows from the fact that the maximum weight matching (not only bipartite instance) form a 2-independence system~\cite{KH78} for which greedy is guarantee to return a 2-approximate solution.

	For the tightness, consider an instance with 2 slots, 2 ad types, and 2 ads of each ad type. For type $\theta_1$, the discount curve is $\alpha^{(\theta_1)}_1 = 1-\epsilon, \alpha^{(\theta_1)}_2 = 0$, with values $v^{(\theta_1)}_1 = v^{(\theta_1)}_2 = 1$ and for type $\theta_2$, the discounts are $\alpha^{(\theta_2)}_1 = \alpha^{(\theta_2)}_2 = 1$, with values $v^{(\theta_2)}_1 = 1, v^{(\theta_2)}_2 = 0$.
	The optimal allocation is to assign slot $s_1$ to $a^{(\theta_1)}_1$ and assign slot $s_2$ to $a^{(\theta_2)}_1$ for a social welfare of $2-\epsilon$.

	Greedy assigns the first slot to $a^{(\theta_2)}_1$ and after that no additional allocation yields a contribution to social welfare (the remaining highest value ad of type $\theta_2$ has value $0$, and the discount for ads of type $\theta_1$ is $0$). The total welfare achieved is $1$. As $\epsilon \rightarrow 0$, the greedy algorithm obtains $\tfrac12$ of the welfare of the optimal allocation.
\end{proof}


\os{TODO: Define the algorithm that obtains the 2-approx, and computes Myerson prices in $O(m^2)$ time assuming sorted input.
Since the allocation curve is monotone, there is a corresponding pricing rule that yields an incentive compatible auction \cite{M81}.
}

\begin{lemma}
	Allocation curve for greedy is monotone.
\end{lemma}
\begin{proof}
	todo, conclusion, exists an linear-time IC mechanism.
\end{proof}


==> notation.tex <==
% !TEX root = main.tex

\section{Notation}
\label{notation}

\begin{itemize}
    \item $a^\theta_i$ is ad $i$ of type $\theta$. When type is irrelevant (e.g. when iterating over all ads) use $a_i$
    \item There are $k$ ad types, $n$ slots, and $n$ ads per type (total $nk$ ads)
    \item $A^\theta$ is the set of ads of type $\theta$, $A$ the set of all ads
    \item $b^\theta_i$ is the per-event bid of ad $a^\theta_i$. We index ads such that for each type $\theta$ we have $b^\theta_1 \ge b^\theta_2 \ge ...\ge b^\theta_n \ge 0.$
    \item $\alpha^\theta_j$ is the event discount for ads of type $\theta$ for slot $j$. By assumption is an order $\sigma$, such that $\alpha^\theta_{\sigma(1)} \geq \alpha^\theta_{\sigma(2)} \geq ... \geq \alpha^\theta_{\sigma(n)} \geq 0$. Wlog, number the slots such that $\sigma$ is the identity function.
    \item $s_j$ is slot $j$ (in descending order of discounts)
    \item phase $j$, the phase corresponding to including slot $j$ in the matching $M$
    \item matching $M$ a running variable, use $M_j$ as the matching at the end of phase $j$
    \item $u^\theta_i\geq 0$ is the shadow variable for ad $a^\theta_i$. When type is irrelevant (e.g. when iterating over all ads) use $u_i$
    \item $p_j\geq 0$ is the shadow price for slot $s_j$
    \item tight-edge graph $T$. The set of edges between ad $a^\theta_i$ and slot $s_j$, such that $u^\theta_i + p_j = \alpha^\theta_j\cdot b^\theta_i$
    \item Alternating BFS tree $B$
    \item $A^{(M)}$ is the set of ads that appear in matching $M$ ($A^{(M)}$ is also known as the set of \emph{allocated} ads); $A^{(M)}_j$ is the set of ads that appear in matching $M_j$ (which is the set at the end of phase $j$)
    \item Similarly, $A^{(\lnot M)}$ is the set of ads that do not appear in $M$; idem for $A^{(\lnot M)}_j$
    % \item $L\subseteq A^{( M)}$ (and similarly $L_j \subseteq A^{( M)}_j$) is the set that consists of the \emph{lowest} matched ad for each type (since ads in in \emph{descending} order, this corresponds to the highest-index matched ad). If the number of matched ads of type $\theta$ is at least $1$, then $l^\theta$ is the lowest matched ad of type $\theta$.
    % \item $H\subseteq A^{(\lnot M)}$ (and similarly $H_j \subseteq A^{(\lnot M)}_j$) is the set that consists of the \emph{highest} unmatched ad for each type (since ads in in \emph{descending} order, this corresponds to the lowest-index unmatched ad). If the number of unmatched ads of type $\theta$ is at least $1$, then $h^\theta$ is the lowest matched ad of type $\theta$.

\end{itemize}

